Solving infinite-horizon Dec-POMDPs using Finite State Controllers within JESP

This paper looks at solving collaborative planning problems formalized as Decentralized POMDPs (Dec-POMDPs) by searching for Nash equilibria, i.e., situations where each agent's policy is a best response to the other agents' (fixed) policies. While the Joint Equilibrium-based Search for Policies (JESP) algorithm does this in the finite-horizon setting relying on policy trees, we propose here to adapt it to infinite-horizon Dec-POMDPs by using finite state controller (FSC) policy representations. In this article, we (1) explain how to turn a Dec-POMDP with $N-1$ fixed FSCs into an infinite-horizon POMDP whose solution is an $N^\text{th}$ agent best response; (2) propose a JESP variant, called \infJESP, using this to solve infinite-horizon Dec-POMDPs; (3) introduce heuristic initializations for JESP aiming at leading to good solutions; and (4) conduct experiments on state-of-the-art benchmark problems to evaluate our approach.

==> Makefile <==
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'

extended.pdf : extended.tex Makefile
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	-$(LATEXMK) -pdf -deps-out=$(DEPS_DIR)/$@P $<
	./clean-deps.sh $(DEPS_DIR)/$@P

clean :
	rm -f *~
	latexmk -c

veryclean:
	rm -rf *~ .deps *.bbl figures/*.bak
	latexmk -C

